From CNNs to Shift-Invariant Twin Models Based on Complex Wavelets

We propose a novel method to increase shift invariance and prediction accuracy in convolutional neural networks. Specifically, we replace the first-layer combination "real-valued convolutions + max pooling" (RMax) by "complex-valued convolutions + modulus" (CMod), which is stable to translations, or shifts. To justify our approach, we claim that CMod and RMax produce comparable outputs when the convolution kernel is band-pass and oriented (Gabor-like filter). In this context, CMod can therefore be considered as a stable alternative to RMax. To enforce this property, we constrain the convolution kernels to adopt such a Gabor-like structure. The corresponding architecture is called mathematical twin, because it employs a well-defined mathematical operator to mimic the behavior of the original, freely-trained model. Our approach achieves superior accuracy on ImageNet and CIFAR-10 classification tasks, compared to prior methods based on low-pass filtering. Arguably, our approach's emphasis on retaining high-frequency details contributes to a better balance between shift invariance and information preservation, resulting in improved performance. Furthermore, it has a lower computational cost and memory footprint than concurrent work, making it a promising solution for practical implementation.

==> inputs/convkernels.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% AlexNet on ImageNet
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure*}[p]
    \centering
    \begin{subfigure}{\textwidth}
        \centering
        \includegraphics[width=0.35\textwidth]{img/convkernels/AI.PDF}
        \includegraphics[width=0.35\textwidth]{img/convkernels/AI_fft.PDF}
        \caption{
            Standard
        }
    \label{subfig:convkernels_wavealexnet_std}
    \end{subfigure} \\
    \begin{subfigure}{\textwidth}
        \centering
        \includegraphics[width=0.35\textwidth]{img/convkernels/AwyI.PDF}
        \includegraphics[width=0.35\textwidth]{img/convkernels/AwyI_fft.PDF}
        \caption{
            \rmaxact (four bottom rows)
        }
    \end{subfigure} \\
    \begin{subfigure}{\textwidth}
        \centering
        \includegraphics[width=0.35\textwidth]{img/convkernels/AwyI_mod_low.PDF}
        \includegraphics[width=0.35\textwidth]{img/convkernels/AwyI_mod_low_fft.PDF} \vspace{-5pt} \\
        \includegraphics[width=0.35\textwidth]{img/convkernels/AwyI_mod_high.PDF}
        \includegraphics[width=0.35\textwidth]{img/convkernels/AwyI_mod_high_fft.PDF}
        \caption{
            \cmodact (four bottom rows). Spatial domain: real part only
        }
    \end{subfigure}
    \caption{
        AlexNet (ImageNet, no blur pooling).
    }
    \label{fig:convkernels_wavealexnet}
\end{figure*}

\begin{figure*}[p]
    \centering
    \begin{subfigure}{\textwidth}
    \centering
        \includegraphics[width=0.35\textwidth]{img/convkernels/Azh3I.PDF}
        \includegraphics[width=0.35\textwidth]{img/convkernels/Azh3I_fft.PDF}
        \caption{
            Blur
        }
    \end{subfigure} \\
    \begin{subfigure}{\textwidth}
    \centering
        \includegraphics[width=0.35\textwidth]{img/convkernels/AzhwyI.PDF}
        \includegraphics[width=0.35\textwidth]{img/convkernels/AzhwyI_fft.PDF}
        \caption{
            \blurrmaxact (four bottom rows) + Blur
        }
    \end{subfigure} \\
    \begin{subfigure}{\textwidth}
    \centering
        \includegraphics[width=0.35\textwidth]{img/convkernels/AzhwyI_mod_low.PDF}
        \includegraphics[width=0.35\textwidth]{img/convkernels/AzhwyI_mod_low_fft.PDF} \vspace{-5pt} \\
        \includegraphics[width=0.35\textwidth]{img/convkernels/AzhwyI_mod_high.PDF}
        \includegraphics[width=0.35\textwidth]{img/convkernels/AzhwyI_mod_high_fft.PDF}
        \caption{
            \cmodact (four bottom rows) + Blur. Spatial domain: real part only
        }
    \end{subfigure}
    \caption{
        AlexNet with static blur pooling (ImageNet).
    }
    \label{fig:convkernels_wavebluralexnet}
\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ResNet-34 on ImageNet
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure*}[p]
    \centering
    \begin{subfigure}{\textwidth}
    \centering
        \includegraphics[width=0.35\textwidth]{img/convkernels/RI.PDF}
        \includegraphics[width=0.35\textwidth]{img/convkernels/RI_fft.PDF}
        \caption{
            Standard
        }
    \label{subfig:convkernels_waveresnet_std}
    \end{subfigure} \\
    \begin{subfigure}{\textwidth}
    \centering
        \includegraphics[width=0.35\textwidth]{img/convkernels/RwyI.PDF}
        \includegraphics[width=0.35\textwidth]{img/convkernels/RwyI_fft.PDF}
        \caption{
            \rmaxact (three bottom rows)
        }
    \end{subfigure} \\
    \begin{subfigure}{\textwidth}
    \centering
        \includegraphics[width=0.35\textwidth]{img/convkernels/RwyI_mod_low.PDF}
        \includegraphics[width=0.35\textwidth]{img/convkernels/RwyI_mod_low_fft.PDF} \vspace{-5pt} \\
        \includegraphics[width=0.35\textwidth]{img/convkernels/RwyI_mod_high.PDF}
        \includegraphics[width=0.35\textwidth]{img/convkernels/RwyI_mod_high_fft.PDF}
        \caption{
            \cmodact (three bottom rows). Spatial domain: real part only
        }
    \end{subfigure}
    \caption{
        ResNet-34 (ImageNet, no blur pooling).
    }
    \label{fig:convkernels_waveresnet}
\end{figure*}

\begin{figure*}[p]
    \centering
    \begin{subfigure}{\textwidth}
    \centering
        \includegraphics[width=0.35\textwidth]{img/convkernels/Rzh3I.PDF}
        \includegraphics[width=0.35\textwidth]{img/convkernels/Rzh3I_fft.PDF}
        \caption{
            Blur
        }
    \end{subfigure} \\
    \begin{subfigure}{\textwidth}
    \centering
        \includegraphics[width=0.35\textwidth]{img/convkernels/RzhwyI.PDF}
        \includegraphics[width=0.35\textwidth]{img/convkernels/RzhwyI_fft.PDF}
        \caption{
            \blurrmaxact (three bottom rows) + Blur
        }
    \end{subfigure} \\
    \begin{subfigure}{\textwidth}
    \centering
        \includegraphics[width=0.35\textwidth]{img/convkernels/RzhwyI_mod_low.PDF}
        \includegraphics[width=0.35\textwidth]{img/convkernels/RzhwyI_mod_low_fft.PDF} \vspace{-5pt} \\
        \includegraphics[width=0.35\textwidth]{img/convkernels/RzhwyI_mod_high.PDF}
        \includegraphics[width=0.35\textwidth]{img/convkernels/RzhwyI_mod_high_fft.PDF}
        \caption{
            \cmodact (three bottom rows) + Blur. Spatial domain: real part only
        }
    \end{subfigure}
    \caption{
        ResNet-34 with static blur pooling (ImageNet).
    }
    \label{fig:convkernels_waveblurresnet}
\end{figure*}

\begin{figure*}[p]
    \centering
    \begin{subfigure}{\textwidth}
    \centering
        \includegraphics[width=0.35\textwidth]{img/convkernels/Rzo3I.PDF}
        \includegraphics[width=0.35\textwidth]{img/convkernels/Rzo3I_fft.PDF}
        \caption{
            ABlur
        }
    \end{subfigure} \\
    \begin{subfigure}{\textwidth}
    \centering
        \includegraphics[width=0.35\textwidth]{img/convkernels/Rzo3wyI.PDF}
        \includegraphics[width=0.35\textwidth]{img/convkernels/Rzo3wyI_fft.PDF}
        \caption{
            \adablurrmaxact (three bottom rows) + ABlur
        }
    \end{subfigure} \\
    \begin{subfigure}{\textwidth}
    \centering
        \includegraphics[width=0.35\textwidth]{img/convkernels/Rzo3wyI_mod_low.PDF}
        \includegraphics[width=0.35\textwidth]{img/convkernels/Rzo3wyI_mod_low_fft.PDF} \vspace{-5pt} \\
        \includegraphics[width=0.35\textwidth]{img/convkernels/Rzo3wyI_mod_high.PDF}
        \includegraphics[width=0.35\textwidth]{img/convkernels/Rzo3wyI_mod_high_fft.PDF}
        \caption{
            \cmodact (three bottom rows) + ABlur. Spatial domain: real part only
        }
    \end{subfigure}
    \caption{
        ResNet-34 with adaptive blur pooling (ImageNet).
    }
    \label{fig:convkernels_waveadablurresnet}
\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ResNet-18 on CIFAR-10
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure*}[p]
    \centering
    \begin{subfigure}{\textwidth}
    \centering
        \includegraphics[width=0.35\textwidth]{img/convkernels/R18C.PDF}
        \includegraphics[width=0.35\textwidth]{img/convkernels/R18C_fft.PDF}
        \caption{
            Standard
        }
    \end{subfigure} \\
    \begin{subfigure}{\textwidth}
    \centering
        \includegraphics[width=0.35\textwidth]{img/convkernels/R18wyC.PDF}
        \includegraphics[width=0.35\textwidth]{img/convkernels/R18wyC_fft.PDF}
        \caption{
            \rmaxact (three bottom rows)
        }
    \end{subfigure} \\
    \begin{subfigure}{\textwidth}
    \centering
        \includegraphics[width=0.35\textwidth]{img/convkernels/R18wyC_mod_low.PDF}
        \includegraphics[width=0.35\textwidth]{img/convkernels/R18wyC_mod_low_fft.PDF} \vspace{-5pt} \\
        \includegraphics[width=0.35\textwidth]{img/convkernels/R18wyC_mod_high.PDF}
        \includegraphics[width=0.35\textwidth]{img/convkernels/R18wyC_mod_high_fft.PDF}
        \caption{
            \cmodact (three bottom rows). Spatial domain: real part only
        }
    \end{subfigure}
    \caption{
        ResNet-18 (CIFAR-10, no blur pooling).
    }
    \label{fig:convkernels_waveresnet_cifar}
\end{figure*}

\begin{figure*}[p]
    \centering
    \begin{subfigure}{\textwidth}
    \centering
        \includegraphics[width=0.35\textwidth]{img/convkernels/R18zh3C.PDF}
        \includegraphics[width=0.35\textwidth]{img/convkernels/R18zh3C_fft.PDF}
        \caption{
            Blur
        }
    \end{subfigure} \\
    \begin{subfigure}{\textwidth}
    \centering
        \includegraphics[width=0.35\textwidth]{img/convkernels/R18zh3wyC.PDF}
        \includegraphics[width=0.35\textwidth]{img/convkernels/R18zh3wyC_fft.PDF}
        \caption{
            \blurrmaxact (three bottom rows) + Blur
        }
    \end{subfigure} \\
    \begin{subfigure}{\textwidth}
    \centering
        \includegraphics[width=0.35\textwidth]{img/convkernels/R18zh3wyC_mod_low.PDF}
        \includegraphics[width=0.35\textwidth]{img/convkernels/R18zh3wyC_mod_low_fft.PDF} \vspace{-5pt} \\
        \includegraphics[width=0.35\textwidth]{img/convkernels/R18zh3wyC_mod_high.PDF}
        \includegraphics[width=0.35\textwidth]{img/convkernels/R18zh3wyC_mod_high_fft.PDF}
        \caption{
            \cmodact (three bottom rows) + Blur. Spatial domain: real part only
        }
    \end{subfigure}
    \caption{
        ResNet-18 with static blur pooling (CIFAR-10).
    }
    \label{fig:convkernels_waveblurresnet_cifar}
\end{figure*}

\begin{figure*}[p]
    \centering
    \begin{subfigure}{\textwidth}
    \centering
        \includegraphics[width=0.35\textwidth]{img/convkernels/R18zo3C.PDF}
        \includegraphics[width=0.35\textwidth]{img/convkernels/R18zo3C_fft.PDF}
        \caption{
            ABlur
        }
    \end{subfigure} \\
    \begin{subfigure}{\textwidth}
    \centering
        \includegraphics[width=0.35\textwidth]{img/convkernels/R18zo3wyC.PDF}
        \includegraphics[width=0.35\textwidth]{img/convkernels/R18zo3wyC_fft.PDF}
        \caption{
            \adablurrmaxact (three bottom rows) + ABlur
        }
    \end{subfigure} \\
    \begin{subfigure}{\textwidth}
    \centering
        \includegraphics[width=0.35\textwidth]{img/convkernels/R18zo3wyC_mod_low.PDF}
        \includegraphics[width=0.35\textwidth]{img/convkernels/R18zo3wyC_mod_low_fft.PDF} \vspace{-5pt} \\
        \includegraphics[width=0.35\textwidth]{img/convkernels/R18zo3wyC_mod_high.PDF}
        \includegraphics[width=0.35\textwidth]{img/convkernels/R18zo3wyC_mod_high_fft.PDF}
        \caption{
            \cmodact (three bottom rows) + ABlur. Spatial domain: real part only
        }
    \end{subfigure}
    \caption{
        ResNet-18 with adaptive blur pooling (CIFAR-10).
    }
    \label{fig:convkernels_waveadablurresnet_cifar}
\end{figure*}
